Embedding Temporal Convolutional Networks for Energy-Efficient PPG-Based Heart Rate Monitoring

Photoplethysmography (PPG) sensors allow for non-invasive and comfortable heart-rate (HR) monitoring, suitable for compact wrist-worn devices. Unfortunately, Motion Artifacts (MAs) severely impact the monitoring accuracy, causing high variability in the skin-to-sensor interface. Several data fusion techniques have been introduced to cope with this problem, based on combining PPG signals with inertial sensor data. Until know, both commercial and reasearch solutions are computationally efficient but not very robust, or strongly dependent on hand-tuned parameters, which leads to poor generalization performance. % In this work, we tackle these limitations by proposing a computationally lightweight yet robust deep learning-based approach for PPG-based HR estimation. Specifically, we derive a diverse set of Temporal Convolutional Networks (TCN) for HR estimation, leveraging Neural Architecture Search (NAS). Moreover, we also introduce ActPPG, an adaptive algorithm that selects among multiple HR estimators depending on the amount of MAs, to improve energy efficiency. We validate our approaches on two benchmark datasets, achieving as low as 3.84 Beats per Minute (BPM) of Mean Absolute Error (MAE) on PPGDalia, which outperforms the previous state-of-the-art. Moreover, we deploy our models on a low-power commercial microcontroller (STM32L4), obtaining a rich set of Pareto optimal solutions in the complexity vs. accuracy space.

==> sections/00_abstract_old.tex <==
\begin{abstract}
%
Wrist-worn wearable devices coupled with photoplethysmography (PPG) sensors allow for non-invasive and comfortable heart-rate (HR) monitoring, albeit with lower accuracy compared to an Electriocardiogram (ECG).
%
However, Motion Artifacts (MAs) can cause a dramatic degradation of the monitoring performance, demanding dedicated and often time-consuming techniques for their removal.
%
Recent state-of-the-art algorithms couple PPG with inertial sensors to mitigate the effect of MAs, but often suffer from poor generalization performance and strong dependence on hand-tuned hyper-parameters. 
%
Moreover, their deployment on MCU-based edge nodes has not been investigated. 
%
Conversely, commercial devices such as Apple Watch and Fitbit use lighter algorithm, which suffer from lower accuracy and higher delays in detecting HR changes.

In this work, we tackle these limitations by proposing a hardware-friendly yet accurate system for PPG-based HR estimation based on Temporal Convolutional Networks (TCN).
%
We introduce a rich family of TCNs, which we call TimePPG, derived from a single ``seed'' model, leveraging an automatic Neural Architecture Search (NAS) approach. 
%
Further, we propose ActPPG, a framework to adaptively combine multiple of such HR estimation models by employing an additional human activity classifier, which assigns samples with limited MAs to a lighter but less accurate HR tracking model, while windows more affected by MAs are tracked by a more accurate (and complex) TCN.
%
On the popular PPGDalia dataset, both the individual models and the ActPPG framework, followed by smoothing post-processing and fine-tuning steps, reach performance levels that outperform the state-of-the-art.
%
% , achieving as low as 3.84 Beats per Minute (BPM) of Mean Absolute Error (MAE).
%
Moreover, deploying ActPPG on an embedded system based on a commercial microcontroller (MCU), the STM32WB55, we obtain a rich set of Pareto architectures in the Complexity vs. accuracy space. Our most accurate implementation reaches 4.88 Beats Per Minute (BPM) of Mean Absolute Error (MAE) - 3.84 BPM with fine-tuning - with a latency of \unit[1.60]{s} and consuming \unit[40.0]{mJ} per inference. At the other extreme, we obtain a MAE of 7.52 BPM with an energy consumption of just \unit[0.29]{mJ}.
%
Compared to other deep learning approaches, one of our Pareto solutions can simultaneously reduce the number of operations by 690$\times$ and the MAE from 8.82 BPM to 5.63 BPM.Photoplethysmography (PPG) sensors allow for non-invasive and comfortable heart-rate (HR) monitoring, suitable for wirst-worn devices in optimized form factor. Unfortunately, Motion Artifacts (MAs) severely impact on the monitoring performance, since they cause high variability in the skin-to-sensor interface. Commercial devices, such as Apple Watch or Fitbit, integrates PPG measure with inertial data, to detect user’ high movements and introduce higher filtering and signals integration. This approach, even computationally efficient, suffer from high delays in the HR detection without ensuring significant accuracy improvement. Recently, several novel data fusion techniques, based on combining PPG signals with inertial sensors were introduced to mitigate the effect of MAs. Such techniques reach a significant reduction in the HR measurement errors, even though they are computationally intensive and  strongly dependent on hand-tuned hyper-parameters, which lead to poor generalization performance and hamper their deployment on low power processors. In this work, we tackle these limitations by proposing a hardware-friendly framework for PPG-based HR estimation based on Temporal Convolutional Networks (TCN), derived from a single ``seed'' model, leveraging an automatic Neural Architecture Search (NAS) approach. Furthermore, we introduce ActPPG, an adaptive algorithm for energy efficient HR estimation, based on the datafusion between PPG and IMU. We validate our approaches on the benchmark PPGDalia dataset, achieving as low as 3.84 Beats per Minute (BPM) of Mean Absolute Error (MAE), which is beyond SoA solutions presented in literature. Finally, we tested the aforementioned approaches on a low power commercial microcontroller, obtaining a rich set of Pareto architectures in the complexity vs. accuracy space. Our most accurate implementation reaches 4.88 Beats Per Minute (BPM) of Mean Absolute Error (MAE) - 3.84 BPM with fine-tuning - with a latency of \unit[1.60]{s} and consuming \unit[40.0]{mJ} per inference. At the other extreme, we obtain a MAE of 7.52 BPM with an energy consumption of just \unit[0.29]{mJ}. 
\end{abstract}

==> sections/Table3.tex <==
\begin{table}
\centering
\caption{MAE of the three algorithms divided by daily activities.}
\label{tab:act_mae}
\begin{tabular}{l|l|l|l}
             & RM {[}BPM{]} & TCNSmall {[}BPM{]} & TCNBig {[}BPM{]} \\ \hline \hline
Transitions (0)  & 12.40        & 6.50               & 6.01             \\
Sitting (1)      & 3.62         & 2.91               & 2.03             \\
Stairs (2)       & 22.77        & 17.39              & 15.96            \\
Table Soccer (3) & 14.82        & 6.54               & 5.09             \\
Cycling (4)      & 21.62        & 8.21               & 6.96             \\
Driving (5)      & 8.08         & 3.44               & 2.76             \\
Launch (6)       & 7.95         & 3.70               & 2.91             \\
Walking (7)      & 14.18        & 7.57               & 7.66             \\
Working (8)      & 6.46         & 2.92               & 2.23             \\ \hline
\end{tabular}
  \vspace{-0.5cm}
\end{table}

==> sections/Table_powers_hardware.tex <==
%
\begin{table}[!t]
%I think some key parameters can be listed, and others can refer to the datasheet
    \caption{Board components power profile. A V$_{DD}$ of 3.3V with a 90\% efficiency is used for the whole board, while a dedicated $V^{MAX30101}_{DD}$ of 5V with 80\% efficiency is used for the MAX30101.}
    \centering
    \label{tab:cpuemodel}
    %\centering
    %\resizebox{\columnwidth}{!}{
        \begin{tabular}{l|l|l|l}
        Component & State & Current (I) & Power Consumption \\
            \hline\hline
            \multicolumn{4}{l}{\textbf{Microcontroller}}\\\hline
            STM32 & Active & 7.59~mA & 25~mW \\ 
            STM32 & Idle & 4.15~mA & 13.7~mW \\
            STM32 & Stop & $2.45~\mu$A & $8.1~\mu W$ \\
            STM32 & BLE$^*$ & $30~\mu A$ & $99~\mu W$\\
            STM32 & BLE$^{\bowtie}$ & $2.1~mA$ & $6.9~mW$\\
            \hline
            \multicolumn{4}{l}{\textbf{Sensors}}\\\hline
            MAX30101 & Active & $1100~\mu A$ & $5.5~mW$ \\
            MAX30101 & Shutdown & $0.7~\mu A$ & $3.5~\mu W$ \\
            LSM6DS & Active & $9~\mu A$ & $30~\mu W$ \\
            LSM6DS & Shutdown & $3~\mu A$ & $10~\mu W$ \\
            \hline\hline
            \multicolumn{4}{l}{$^*$  STM32 BLE current advertising (0~dBm; 1~s; 31~B).}\\ 
            \multicolumn{4}{l}{$^{\bowtie}$  STM32 BLE  connected master (200~B; 100~ms)} 
        \end{tabular}
  \vspace{-0.5cm}
    %}
\end{table}
%
